AgentSimulator: An Agent-based Approach for Data-driven Business Process Simulation

Business process simulation (BPS) is a versatile technique for estimating process performance across various scenarios. Traditionally, BPS approaches employ a control-flow-first perspective by enriching a process model with simulation parameters. Although such approaches can mimic the behavior of centrally orchestrated processes, such as those supported by workflow systems, current control-flow-first approaches cannot faithfully capture the dynamics of real-world processes that involve distinct resource behavior and decentralized decision-making. Recognizing this issue, this paper introduces AgentSimulator, a resource-first BPS approach that discovers a multi-agent system from an event log, modeling distinct resource behaviors and interaction patterns to simulate the underlying process. Our experiments show that AgentSimulator achieves state-of-the-art simulation accuracy with significantly lower computation times than existing approaches while providing high interpretability and adaptability to different types of process-execution scenarios.

==> Tables/motivation_log.tex <==
% \begin{table}[t]
% \centering
% \setlength\tabcolsep{6pt} % default value: 6pt
% \caption{Subset of a simple event log.}
% \label{tab:example_log}
% \begin{tabular}{ccccc}
% \hline
% \toprule
% \textbf{Caseid} & \textbf{Activity} & \textbf{Start} & \textbf{End} & \textbf{Agent}  \\ 
% \midrule
%  1 & A & 30-05-24 08:00 & 30-05-24 08:30 & 1 \\ 
%  2 & A & 30-05-24 08:10 & 30-05-24 08:15 & 2 \\
%  2 & B & 30-05-24 08:15 & 30-05-24 08:15 & 3 \\
%  2 & C & 30-05-24 08:20 & 30-05-24 08:40 & 1 \\
%  1 & B & 30-05-24 08:30 & 30-05-24 08:30 & 3 \\
%  1 & C & 30-05-24 08:30 & 30-05-24 08:50 & 2 \\

%  \hline
% \end{tabular}
% \end{table}

\begin{table}[t]
\centering
\setlength\tabcolsep{2pt} % default value: 6pt
\caption{Subset of a simple event log.}
\label{tab:example_log}
\begin{tabular}{lllll}
\hline
\toprule
\textbf{Caseid} & \textbf{Activity} & \textbf{Start} & \textbf{End} & \textbf{Resource}  \\ 
\midrule
 1 & Application received & 30-05-24 08:00 & 30-05-24 08:00 & System \\ 
 1 & Check credit history & 30-05-24 08:00 & 30-05-24 08:45 & Steve \\
 1 & Check income sources & 30-05-24 08:45 & 30-05-24 09:00 & Oliver \\
 1 & Assess application & 30-05-24 09:00 & 30-05-24 09:20 & Maria \\
 1 & Notify customer & 30-05-24 09:20 & 30-05-24 09:25 & Maria \\
 2 & Application received & 30-05-24 08:50 & 30-05-24 08:50 & System \\
 2 & Check credit history & 30-05-24 08:50 & 30-05-24 09:10 & Angela \\
 
 2 & Check income sources & 30-05-24 09:10 & 30-05-24 09:30 & Angela \\
 
 2 & Assess application & 30-05-24 09:30 & 30-05-24 09:50 & Patrick \\
 2 & Notify customer & 30-05-24 09:50 & 30-05-24 09:55 & Patrick \\
 3 & Application received & 30-05-24 09:30 & 30-05-24 09:30 & System \\ 
 3 & Check credit history & 30-05-24 09:30 & 30-05-24 09:45 & Oliver \\
 3 & Check income sources & 30-05-24 09:45 & 30-05-24 10:30 & Steve \\
 
 \vdots & \vdots & \vdots & \vdots & \vdots \\

 \hline
\end{tabular}
\end{table}

==> Tables/run_time.tex <==
\begin{table}[t]
\centering
\setlength\tabcolsep{4pt} % default value: 6pt
\caption{Comparison of run times in minutes across different simulators.}
\label{tab:run_time}
\begin{tabular}{cccccc}
\hline
\toprule
\textbf{Log} & \textbf{Simod} & \textbf{DGEN} & \textbf{DSIM} & \textbf{AgentSimulator} \\ 
\midrule
 Loan Application & 8.7  & 0 & 0 & 1.5 \\ 
 P2P & 0  & 0 & 0 & 0 \\ 
 CVS & 0  & 0 & 0 & 0 \\ 
 Confidential 1000 & 0  & 0 & 0 & 7.25 \\ 
 Confidential 2000 & 0  & 0 & 0 & 0\\ 
 ACR & 0  & 0 & 0 & 0 \\ 
 Production & 0  & 0 & 0 & 0.33 \\ 
 BPI12W & 15.8  & 0 & 0 & 0 \\ % 100 logs takes 21 minutes
 BPI17W & 0  & 0 & 0 & 0 \\ 

 \hline
\end{tabular}
\end{table}
